Stability to Deformations of Manifold Filters and Manifold Neural Networks

The paper defines and studies manifold (M) convolutional filters and neural networks (NNs). \emph{Manifold} filters and MNNs are defined in terms of the Laplace-Beltrami operator exponential and are such that \emph{graph} (G) filters and neural networks (NNs) are recovered as discrete approximations when the manifold is sampled. These filters admit a spectral representation which is a generalization of both the spectral representation of graph filters and the frequency response of standard convolutional filters in continuous time. The main technical contribution of the paper is to analyze the stability of manifold filters and MNNs to smooth deformations of the manifold. This analysis generalizes known stability properties of graph filters and GNNs and it is also a generalization of known stability properties of standard convolutional filters and neural networks in continuous time. The most important observation that follows from this analysis is that manifold filters, same as graph filters and standard continuous time filters, have difficulty discriminating high frequency components in the presence of deformations. This is a challenge that can be ameliorated with the use of manifold, graph, or continuous time neural networks. The most important practical consequence of this analysis is to shed light on the behavior of graph filters and GNNs in large-scale graphs.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> suplement.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% SUBSECTION %%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\setcounter{subsection}{0}

\subsection{Proof of Proposition \ref{prop:finite_num}}
\label{sup:weyl}
Weyl's law in \cite{musser2016weyl} states that if $\ccalM$ is a compact connected oriented Riemannian manifold of dimension $d$ then 
\begin{equation}\label{eqn:weylslaw-musser}
    N(\lambda)\sim \frac{C_d}{(2\pi)^d}Vol(\ccalM) \lambda^{d/2}\text{ with } N(\lambda):=\#\{\lambda_k\leq \lambda\}.
\end{equation}
Since eigenvalues of the LB operator $\ccalL$ are $0<\lambda_1\leq \lambda_2\leq \lambda_3\cdots$  repeated according to its multiplicity, we can have
\begin{equation}\label{eqn:weylslaw}
\lambda_k \sim \frac{(2\pi)^2}{(C_d Vol(\ccalM))^{2/d}}k^{2/d},
\end{equation}
where $C_d$ denotes the volume of the unit ball of $\reals^d$ and $Vol(\ccalM)$ is the volume of manifold $\ccalM$. This indicates that $\lambda_k$ grows with the same order of the magnitude with $\frac{(2\pi)^2}{(C_d Vol(\ccalM))^{2/d}}k^{2/d}$. With this asymptotic equivalence relationship, we can have
\begin{align}
  &  \lambda_{k+1} -\frac{(2\pi)^2(k+1)^{2/d}}{(C_d Vol(\ccalM))^{2/d}} = o\left(\frac{(2\pi)^2(k+1)^{2/d}}{(C_d Vol(\ccalM))^{2/d}}\right),\\
   & \frac{(2\pi)^2}{(C_d Vol(\ccalM))^{2/d}}k^{2/d} - \lambda_k = o(\lambda_k)
\end{align}
Therefore, for any constant $C_1>0$, we can find some $K_1(C_1)>0$, which indicates that $K_1$ depends on $C_1$, such that for all $k>K_1(C_1)$, we have
\begin{equation}
\label{eq:lambda_k+1}
     \lambda_{k+1} -\frac{(2\pi)^2(k+1)^{2/d}}{(C_d Vol(\ccalM))^{2/d}} <  \frac{C_1(2\pi)^2(k+1)^{2/d}}{(C_d Vol(\ccalM))^{2/d}}.
\end{equation}
Similarly, for any constant $C_2>0$, we can find some $K_2(C_2)>0$, such that for all $k>K_2(C_2)$, we have
\begin{equation}
\label{eq:lambda_k}
    \frac{(2\pi)^2}{(C_d Vol(\ccalM))^{2/d}}k^{2/d} - \lambda_k < C_2 \lambda_k.
\end{equation}
Therefore from \eqref{eq:lambda_k+1} and \eqref{eq:lambda_k} we can get upper and lower bound for $\lambda_{k+1}$ and $\lambda_k$ respectively. If 
\begin{align}
   (1+C_1) (k+1)^{2/d}- \frac{k^{2/d}}{1+C_2}\leq \frac{\alpha (Vol(\ccalM) C_d)^{2/d}}{4\pi^2} ,
\end{align}
we can have $\lambda_{k+1}-\lambda_k\leq \alpha$. The left side can be scaled down to $$(k+1)^{2/d}-k^{2/d}\geq \min\{1+C_1, \frac{1}{1+C_2}\}\frac{2}{d}k^{2/d-1} = \frac{C_0}{d}k^{2/d-1}$$ This implies that 
\begin{align}
    k \geq  \left( \frac{\alpha d (Vol(\ccalM) C_d)^{2/d}}{C_04\pi^2} \right)^{\frac{d}{2-d}},
\end{align}
with $d>2$, we can claim that for all $k > K_0(C_0) = \max\{K_1(C_1), K_2(C_2)\}$, if $k$ satisfies
$$k\geq  \Big\lceil \left(\frac{\alpha d}{C_04\pi^2}\right)^{d/(2-d)}(C_d \text{Vol}(\ccalM))^{2/(2-d)} \Big\rceil,$$ it holds that $\lambda_{k+1}-\lambda_k\leq \alpha$. Proof of Proposition \ref{prop:finite_num_rela} is similar and is also based on \eqref{eqn:weylslaw}.

 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% SUBSECTION %%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  \subsection{Proof of Theorem \ref{thm:stability_nn_rela}}
%  \label{app:stability_nn_rela}
%  For the stability of MNN with $\gamma$-FRT filters, the result can be derived with the same routine but replace the $C_{per}$ term as $C_{per}= \frac{M_s\pi}{\gamma-\epsilon+\gamma\epsilon}+\frac{2B_h}{2-\epsilon}+\frac{2(M-M_s)\delta}{\epsilon}$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% SUBSECTION %%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% SUBSECTION %%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
 \subsection{Proof of Proposition \ref{prop:convergence}}
 \label{app:convergence}
 Considering that the discrete points $\{x_1,x_2,\hdots,x_n\}$ are uniformly sampled from manifold $\ccalM$ with measure $\mu$, the empirical measure associated with $\text{d}\mu$ can be denoted as $p_n=\frac{1}{n}\sum_{i=1}^n \delta_{x_i}$, where $\delta_{x_i}$ is the Dirac measure supported on $x_i$. Similar to the inner product defined in the $L^2(\ccalM)$ space \eqref{eqn:innerproduct}, the inner product on $L^2(\bbG_n)$ is denoted as
 \begin{equation}
     \langle u, v\rangle_{L^2(\bbG_n)}=\int u(x)v(x)\text{d}p_n=\frac{1}{n}\sum_{i=1}^n u(x_i)v(x_i).
 \end{equation}
 The norm in $L^2(\bbG_n)$ is therefore $\|u\|^2_{L^2(\bbG_n)} = \langle u, u \rangle_{L^2(\bbG_n)}$, with $u,v \in L^2(\ccalM)$. For signals $\bbu,\bbv \in L^2(\bbG_n)$, the inner product is therefore $\langle \bbu,\bbv \rangle_{L^2(\bbG_n)} = \frac{1}{n}\sum_{i=1}^n [\bbu]_i[\bbv]_i$. From here we write $\|\cdot\|_{L^2(\bbG_n)}$ as $\|\cdot\|$ for simplicity.
 
 We first import the existing results from \cite{belkin2006convergence} which indicates the spectral convergence of the constructed Laplacian operator based on the graph $\bbG_n$ to the LB operator of the underlying manifold.
 \begin{theorem}[Theorem 2.1 \cite{belkin2006convergence}]
 \label{thm:convergence}
 Let $X=\{x_1, x_2,...x_n\}$ be a set of $n$ points sampled i.i.d. from a $d$-dimensional manifold $\ccalM \subset \reals^N$. % sampled by an operator $\bbP_n$ \eqref{eqn:sampling}. 
 Let $\bbG_n$ be a graph approximation of $\ccalM$ constructed from $X$ with weight values set as \eqref{eqn:weight} with $t_n = n^{-1/(d+2+\alpha)}$ and $\alpha>0$. Let $\bbL_n$ be the graph Laplacian of $\bbG_n$ and $\ccalL$ be the Laplace-Beltrami operator of $\ccalM$. Let $\lambda_{i}^n$ be the $i$-th eigenvalue of $\bbL_n$ and $\bm\phi_{i}^n$ be the corresponding normalized eigenfunction. Let $\lambda_i$ and $\bm\phi_i$ be the corresponding eigenvalue and eigenfunction of $\ccalL$ respectively. Then, it holds that
\begin{equation}
\label{eqn:convergence_spectrum}
    \lim_{n\rightarrow \infty } \lambda_i^n = \lambda_i, \quad \lim_{n\rightarrow \infty} |\bm\phi^{n}_i(x_j) -  \bm\phi_i(x_j)|=0, j=1,2 \hdots,n
\end{equation}
where the limits are taken in probability.
 \end{theorem}
 

With the definitions of neural networks on graph $\bbG_n$ and manifold $\ccalM$, the output difference can be written as 
 \begin{align}
    \nonumber \|\bm\Phi(\bbH,\bbL_n,\bbP_nf)-\bbP_n \bm\Phi&(\bbH,\ccalL, f))\| = \left\| \sum_{q=1}^{F_L}\bbx_L^q-\sum_{q=1}^{F_L}\bbP_n f_L^q \right\|\\
     & \leq \sum_{q=1}^{F_L} \left\| \bbx_L^q- \bbP_n f_L^q \right\|.
 \end{align}
 By inserting the definitions, we have 
 \begin{align}
   \nonumber  &\left\| \bbx_l^p- \bbP_n f_l^p \right\|\\
     &=\left\| \sigma\left(\sum_{q=1}^{F_{l-1}} \bbh_l^{pq}(\bbL_n) \bbx_{l-1}^q \right) -\bbP_n \sigma\left(\sum_{q=1}^{F_{l-1}} \bbh_l^{pq}(\ccalL) f_{l-1}^q\right) \right\|
 \end{align}
 with $\bbx_0=\bbP_n f$ as the input of the first layer. With a normalized Lipschitz nonlinearity, we have
  \begin{align}
    \| \bbx_l^p - \bbP_n f_l^p & \| \leq \left\|  \sum_{q=1}^{F_{l-1}} \bbh_l^{pq}(\bbL_n) \bbx_{l-1}^q    - \bbP_n \sum_{q=1}^{F_{l-1}} \bbh_l^{pq}(\ccalL)  f_{l-1}^q\right\|\\
    & \leq \sum_{q=1}^{F_{l-1}} \left\|    \bbh_l^{pq}(\bbL_n) \bbx_{l-1}^q    - \bbP_n   \bbh_l^{pq}(\ccalL)  f_{l-1}^q\right\|
 \end{align}
 The difference can be further decomposed as
\begin{align}
   \nonumber   \|    \bbh_l^{pq}(\bbL_n) & \bbx_{l-1}^q    - \bbP_n   \bbh_l^{pq}(\ccalL)  f_{l-1}^q \| 
   \\ \nonumber&\leq \|
\bbh_l^{pq}(\bbL_n) \bbx_{l-1}^q  - \bbh_l^{pq}(\bbL_n) \bbP_n f_{l-1}^q \\ &\qquad +\bbh_l^{pq}(\bbL_n) \bbP_n f_{l-1}^q  - \bbP_n   \bbh_l^{pq}(\ccalL)  f_{l-1}^q
    \|\\\nonumber
   & \leq \left\|
    \bbh_l^{pq}(\bbL_n) \bbx_{l-1}^q  - \bbh_l^{pq}(\bbL_n) \bbP_n f_{l-1}^q
    \right\|
  \\ &\qquad +
    \left\|
    \bbh_l^{pq}(\bbL_n) \bbP_n f_{l-1}^q  - \bbP_n   \bbh_l^{pq}(\ccalL)  f_{l-1}^q
    \right\|
\end{align}
The first term can be bounded as $\| \bbx_{l-1}^q - \bbP_nf_{l-1}^q\|$ with the initial condition $\|\bbx_0 - \bbP_n f_0\|=0$. The second term can be denoted as $D_{l-1}^n$. With the iteration employed, we can have
\begin{align}
 \nonumber \|\bm\Phi(\bbH,\bbL_n,\bbP_n f) - \bbP_n \bm\Phi(\bbH,\ccalL,f)\| 
 \leq
 \sum_{l=0}^L \prod\limits_{l'=l}^L F_{l'} D_l^n.
 \end{align}
 Therefore, we can focus on the difference term $D_l^n$, we omit the feature and layer index to work on a general form.
  \begin{align}
    &\nonumber \|\bbh(\bbL_n)\bbP_n f - \bbP_n\bbh(\ccalL) f\|\\
    &= \left\| \sum_{i=1}^n \hat{h}(\lambda_i^n) \langle \bbP_nf,\bm\phi_i^n \rangle_{\bbG_n}\bm\phi_i^n - \sum_{i=1}^\infty \hat{h}(\lambda_i)\langle f,\bm\phi_i\rangle_{\ccalM} \bbP_n \bm\phi_i  \right\|
    %  \\ 
    %  &\nonumber \leq  \left\| \sum_{i=1}^M \hat{h}(\lambda_i^n) \langle \bbP_nf,\bm\phi_i^n \rangle_{\bbG_n}\bm\phi_i^n - \sum_{i=1}^M \hat{h}(\lambda_i) \langle \bbP_nf,\bm\phi_i^n \rangle_{\bbG_n}\bm\phi_i^n\right\| \\
    %  & \qquad \qquad \qquad \qquad\qquad \qquad+\left\| \sum_{i=1}^M \hat{h}(\lambda_i) \langle \bbP_n f,\bm\phi_i^n \rangle_{\bbG_n} \bm\phi_i^n - \sum_{i=1}^M \hat{h}(\lambda_i) \langle f,\bm\phi_i \rangle_{\ccalM} \bbP_n \bm\phi_i \right\|.\label{eqn:conv-1}
 \end{align}
 
 We decompose the $\alpha$-FDT filter function as $\hat{h}(\lambda)=h^{(0)}(\lambda)+\sum_{l\in\ccalK_m}h^{(l)}(\lambda)$ as equations \eqref{eqn:h0} and \eqref{eqn:hl} show. With the triangle inequality and $n > N_\alpha=\max_{i}\{\lambda_i\in[\Lambda_k(\alpha)]_{k\in\ccalK_s}\}$, we start by analyzing the output difference of $h^{(0)}(\lambda)$ as
 \begin{align}
    & \nonumber \left\| \sum_{i=1}^{N_\alpha} {h}^{(0)}(\lambda_i^n) \langle \bbP_nf,\bm\phi_i^n \rangle_{\bbG_n}\bm\phi_i^n - \sum_{i=1}^{N_\alpha} {h}^{(0)}(\lambda_i)\langle f,\bm\phi_i\rangle_{\ccalM} \bbP_n \bm\phi_i  \right\|
     \\ 
     &\nonumber \leq  \left\| \sum_{i=1}^{N_\alpha} \left({h}^{(0)}(\lambda_i^n)- {h}^{(0)}(\lambda_i) \right) \langle \bbP_nf,\bm\phi_i^n \rangle_{\bbG_n}\bm\phi_i^n \right\| \\
     &  +\left\| \sum_{i=1}^{N_\alpha} {h}^{(0)}(\lambda_i)\left( \langle \bbP_n f,\bm\phi_i^n \rangle_{\bbG_n} \bm\phi_i^n - \langle f,\bm\phi_i \rangle_{\ccalM} \bbP_n \bm\phi_i \right)  \right\|.\label{eqn:conv-1}
 \end{align}
 
 The first term in \eqref{eqn:conv-1} can be bounded by leveraging the $A_h$-Lipschitz continuity of the frequency response. From the convergence in probability stated in \eqref{eqn:convergence_spectrum}, we can claim that for each eigenvalue $\lambda_i \leq \lambda_{N_\alpha}$, for all $\epsilon_i>0$ and all $\delta_i>0$, there exists some $N_i$ such that for all $n>N_i$, we have
\begin{gather}
 \label{eqn:eigenvalue}   \mathbb{P}(|\lambda_i^n-\lambda_i|\leq \epsilon_i)\geq 1-\delta_i,
 \end{gather}
Letting $\epsilon_i < \epsilon$ with $\epsilon > 0$, with probability at least $\prod_{i=1}^M(1-\delta_i) := 1-\delta$, the first term is bounded as 
 
\begin{align}
   &\nonumber \left\| \sum_{i=1}^{N_\alpha} ({h}^{(0)}(\lambda_i^n) - {h}^{(0)}(\lambda_i)) \langle \bbP_n f,\bm\phi_i^n \rangle_{\bbG_n} \bm\phi_i^n  \right\|\\
   & \leq \sum_{i=1}^{N_\alpha} |{h}^{(0)}(\lambda_i^n)-{h}^{(0)}(\lambda_i)| |\langle \bbP_n f,\bm\phi_i^n \rangle_{\bbG_n}| \|\bm\phi_i^n\|\\
   &\leq \sum_{i=1}^{N_\alpha} A_h |\lambda_i^n-\lambda_i| \|\bbP_n f\| \|\bm\phi_i^n \|^2\leq N_s A_h\epsilon,
\end{align} 
for all $n>\max\{\max_i N_i, N_\alpha\} := N$.

The second term in \eqref{eqn:conv-1} can be bounded combined with the convergence of eigenfunctions in \eqref{eqn:eigenfunction} as
\begin{align}
  & \nonumber \Bigg\| \sum_{i=1}^{N_\alpha}{h}^{(0)}(\lambda_i)\left( \langle \bbP_nf,\bm\phi_i^n \rangle_{\bbG_n}\bm\phi_i^n - \langle f,\bm\phi_i \rangle_{\ccalM} \bbP_n \bm\phi_i\right)  \Bigg\|\\
   & \leq \nonumber \Bigg\|  \sum_{i=1}^{N_\alpha} {h}^{(0)}(\lambda_i)  \left(\langle \bbP_n f,\bm\phi_i^n\rangle_{\bbG_n}\bm\phi_i^n  - \langle \bbP_nf,\bm\phi_i^n \rangle_{\bbG_n} \bbP_n\bm\phi_i\right)\Bigg\|\\
   &\label{eqn:term1}+ \left\| \sum_{i=1}^{N_\alpha}  {h}^{(0)}(\lambda_i) \left(\langle \bbP_n f,\bm\phi_i^n\rangle_{\bbG_n} \bbP_n\bm\phi_i -\langle f,\bm\phi_i\rangle_\ccalM \bbP_n\bm\phi_i \right) \right\|
%   &\leq \nonumber \sum_{i=1}^n \langle \bbP_nf,\bm\phi_i^n \rangle \| \bm\phi_i^n-\bbP_n\bm\phi_i \|\\
%   &\qquad \qquad + \sum_{i=1}^n|\langle \bbP_n f, \bm\phi_i^n\rangle -\langle f,\bm\phi_i\rangle|\left\| \bbP_n\bm\phi_i \right\|
\end{align}
From the convergence stated in \eqref{eqn:convergence_spectrum}, we can claim that for some fixed eigenfunction $\bm\phi_i$,  for all $\epsilon_i>0$ and all $\delta_i>0$, there exists some $N_i$ such that for all $n>N_i$, we have
\begin{gather}
 \label{eqn:eigenfunction}    \mathbb{P}(|\bm\phi_i^n(x_j) - \bm\phi_i(x_j)|\leq \epsilon_i)\geq 1-\delta_i,\quad \forall \; x_j\in X .
 \end{gather}
 Therefore, letting $\epsilon_i < \epsilon$ with $\epsilon > 0$, with probability at least $\prod_{i=1}^M(1-\delta_i) := 1-\delta$, for all $n>\max\{\max_i N_i, N_\alpha\} := N$, the first term in \eqref{eqn:term1} can be bounded as
\begin{align}
& \nonumber \left\|  \sum_{i=1}^{N_\alpha} {h}^{(0)}(\lambda_i) \left(\langle \bbP_n f,\bm\phi_i^n\rangle_{\bbG_n}\bm\phi_i^n  - \langle \bbP_nf,\bm\phi_i^n \rangle_{\ccalM} \bbP_n\bm\phi_i\right)\right\|\\
& \qquad \qquad\leq \sum_{i=1}^{N_\alpha} \|\bbP_n f\|\|\bm\phi_i^n - \bbP_n\bm\phi_i\|\leq N_s \epsilon,
\end{align}
because the frequency response is non-amplifying as stated in Assumption \ref{ass:filter_function}. The last equation comes from the definition of norm in $L^2(\bbG_n)$.
The second term in \eqref{eqn:term1} can be written as
\begin{align}
     & \nonumber \Bigg\| \sum_{i=1}^{N_\alpha}  {h}^{(0)}(\lambda_i^n) (\langle \bbP_n f,\bm\phi_i^n\rangle_{\bbG_n}  \bbP_n\bm\phi_i -\langle f,\bm\phi_i\rangle_\ccalM \bbP_n\bm\phi_i ) \Bigg\| \\
   &\leq \sum_{i=1}^{N_\alpha} |{h}^{(0)}(\lambda_i^n)| \left|\langle \bbP_n f,\bm\phi_i^n\rangle_{\bbG_n}  -\langle f,\bm\phi_i\rangle_\ccalM\right|\|\bbP_n\bm\phi_i\|.
\end{align}
Because $\{x_1, x_2,\cdots,x_n\}$ is a set of uniform sampled points from $\ccalM$, based on Theorem 19 in \cite{von2008consistency} we can claim that there exists some $N$ such that for all $n>N$
\begin{equation}
   \mathbb{P}\left(\left|\langle \bbP_n f,\bm\phi_i^n\rangle_{\bbG_n}  -\langle f,\bm\phi_i\rangle_\ccalM\right|\leq\epsilon \right)\geq 1-\delta,
\end{equation}
for all $\epsilon>0$ and $\delta>0$. Taking into consider the boundedness of frequency response $|{h}^{(0)}(\lambda)|\leq 1$ and the bounded energy $\|\bbP_n\bm\phi_i\|$. Therefore, we have for all $\epsilon>0$ and $\delta>0$,
\begin{align}
&\nonumber  \mathbb{P}\left(\left\| \sum_{i=1}^{N_\alpha}  h^{(0)}(\lambda_i^n) \left(\langle \bbP_n f,\bm\phi_i^n\rangle_{\bbG_n}  -\langle f,\bm\phi_i\rangle_\ccalM \right)\bbP_n\bm\phi_i  \right\|\leq N_s \epsilon\right)
\\& \qquad \qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad\geq 1-\delta,
\end{align}
for all $n>N$.

Combining the above results, we can bound the output difference of $h^{(0)}(\lambda)$. Then we need to analyze the output difference of $h^{(l)}(\lambda)$ and bound this as
\begin{align}
    \nonumber &\left\| \bbP_n \bbh^{(l)}(\ccalL)f -\bbh^{(l)}(\bbL_n)\bbP_n f \right\| 
    \\& \leq \left\| (\hat{h}(C_l)+\delta)\bbP_n f - (\hat{h}(C_l)-\delta)\bbP_nf\right\| \leq 2\delta\|\bbP_nf\|,
\end{align}
where $\bbh^{(l)}(\ccalL)$ and $\bbh^{(l)}(\bbL_n)$ are filters with filter function $h^{(l)}(\lambda)$ on the LB operator $\ccalL$ and graph Laplacian $\bbL_n$ respectively.
Combining the filter functions, we can write
\begin{align}
   \nonumber &\|\bbP_n\bbh(\ccalL)f-\bbh(\bbL_n)\bbP_n f\|\\\nonumber &=
    \Bigg\|\bbP_n\bbh^{(0)}(\ccalL)f +\bbP_n\sum_{l\in\ccalK_m}\bbh^{(l)}(\ccalL)f -\\& \qquad \qquad \qquad \bbh^{(0)}(\bbL_n)\bbP_n f - \sum_{l\in\ccalK_m} \bbh^{(l)}(\bbL_n)\bbP f \Bigg\|\\
    &\nonumber \leq \|\bbP_n \bbh^{(0)}(\ccalL)f-\bbh^{(0)}(\bbL_n)\bbP_n f\|+\\
    &\qquad \qquad \qquad \sum_{l\in\ccalK_m}\|\bbP_n \bbh^{(l)}(\ccalL)f-\bbh^{(l)}(\bbL_n)\bbP_nf\|.
\end{align}


Above all, we can claim that there exists some $N$, such that for all $n>N$, for all $\epsilon'>0$ and $\delta>0$, we have
\begin{equation}
    \mathbb{P}(\|\bbh(\bbL_n)\bbP_n f - \bbP_n\bbh(\ccalL) f\|\leq \epsilon')\geq 1-\delta.
\end{equation}




With $\lim\limits_{n\rightarrow \infty}D_l^n=0$ in high probability, this concludes the proof. 
